Khronos: A Unified Approach for Spatio-Temporal Metric-Semantic SLAM in Dynamic Environments

Perceiving and understanding highly dynamic and changing environments is a crucial capability for robot autonomy. While large strides have been made towards developing dynamic SLAM approaches that estimate the robot pose accurately, a lesser emphasis has been put on the construction of dense spatio-temporal representations of the robot environment. A detailed understanding of the scene and its evolution through time is crucial for long-term robot autonomy and essential to tasks that require long-term reasoning, such as operating effectively in environments shared with humans and other agents and thus are subject to short and long-term dynamics. To address this challenge, this work defines the Spatio-temporal Metric-semantic SLAM (SMS) problem, and presents a framework to factorize and solve it efficiently. We show that the proposed factorization suggests a natural organization of a spatio-temporal perception system, where a fast process tracks short-term dynamics in an active temporal window, while a slower process reasons over long-term changes in the environment using a factor graph formulation. We provide an efficient implementation of the proposed spatio-temporal perception approach, that we call Khronos, and show that it unifies exiting interpretations of short-term and long-term dynamics and is able to construct a dense spatio-temporal map in real-time. We provide simulated and real results, showing that the spatio-temporal maps built by Khronos are an accurate reflection of a 3D scene over time and that Khronos outperforms baselines across multiple metrics. We further validate our approach on two heterogeneous robots in challenging, large-scale real-world environments.

==> sections/drafts.tex <==


\section{Problem Statement} 
\label{sec:problem}

\todo[LS]{This page will be updated to be essentially current Sec. IV.A/B}

\parsec{World Model}
Consider an area of interest $\mathcal{W}$, which is a bounded region of space and time $\mathcal{W} \subseteq \mathbb{R}^3 \times \mathbb{R}^{+}$.
The area has an observable state $\Omega(t)$ at time $t$. At each frame $t$, the robot takes a measurement $_SP^t$ in sensor frame $S$: 
\begin{gather}
    _SP^{(t)} \sim _S\bar{\Omega}(t) + \epsilon 
\end{gather}
where $\epsilon$ is the sensing noise and $\bar{\Omega}(t) \subseteq \Omega$(t) is the part of $\Omega$ observed in frame $t$.
In this task, $\Omega$ denotes all surfaces in $\mathcal{W}$\footnote{
\LC{for ICRA, I suggest keeping things more grounded, and then trying to be slightly more general in a followup journal-- I would remove this for now}
Without loss of generality, $\Omega$ could also include e.g. smells, temperature or other observables in other cases.}. 

% -----------------------------------------------------------------------------------------------
% \parsec{Assumptions}
% We assume there exists a discrete structure of objects $\mathcal{O}$ that gives rise to $\Omega$:
% \begin{gather}
%     \exists \mathcal{O} = \{ o_i \},\quad o_i = \{_{O_i}\Omega_i,\ T_{WO_i} \} \quad \text{s.t.} \\
%     _W\Omega = \sum_\mathcal{O} T_{WO_i}*_{O_i}\Omega_i \label{eq:composition}
% \end{gather}

% -----------------------------------------------------------------------------------------------
\parsec{Metric Semantic Mapping}
The goal is to estimate a map $M$, as a discrete structure of objects ${o_j}$ that gives rise to $\Omega$:
\begin{gather}
    M = \{ o_i \},\quad o_i = \{_{O_i}\Omega_i,\ T_{WO_i} \} \quad \text{s.t.} \\
    _W\Omega = \sum_\mathcal{E} T_{WE_i}*_{E_i}\Omega_i \label{eq:composition}
\end{gather}
\LC{E should be O?}
\LC{the second relation might only be satisfied up to noise. also what about the background?}
Each object $o_i$ has a surface $\Omega_i$, and a transformation w.r.t. to the world $T_{WO_i}$.
The world is completely represented by all element surfaces (\ref{eq:composition}).
\todo{elements / objects? Define objects as surfaces that move consistently/coherently together for this project. This property is practically also relevant for e.g. manipulation tasks. }
\note{Continuity constraints on the temporal evolution of everything? This might be useful for long-term short-term. }

% -----------------------------------------------------------------------------------------------
\parsec{Dynamic World}
In general, all parts may be dynamic. This includes: objects may move over time (\ref{eq:ob_move}), objects may be deformable (\ref{eq:ob_deformable}), the underlying structure is an open (changing) set (\ref{eq:ob_change}):
\begin{gather}
    T_{WO_i} = T_{WO_i}(t) \label{eq:ob_move} \\
    \Omega_i = \Omega_i(t) \label{eq:ob_deformable} \\
    \mathcal{O} = \mathcal{O}(t) \label{eq:ob_change} \\
    _W\Omega(t) = \sum_{\mathcal{O}(t)} T_{OE_i}(t) * _{O_i}\Omega_i(t)
\end{gather}

In this work, we limit the scope to the cases where objects are rigid $\Omega_i = const$. \note{although we deal with deforming humans, we don't represent them or other deforming objects / it's fair to say it's not a focus}.

% -----------------------------------------------------------------------------------------------
\parsec{Spatio-temporal Metric Semantic Mapping}
\LC{I agree with the discussion so far, which essentially introduces the variables we care about. But at this point I suggest phrasing things probabilistically as we did on the board. currently, eq (15) seems heuristic and instead it would be nice for it to fall out of the probabilistic derivation}
The goal is to estimate the best possible spatio-temporal map $M^\star_t(t')$ incrementally at time $t$, explaining all previous times $t' \leq t$:

\begin{equation}
    M^\star_t(t') = \min_{M(t')} \int_0^t \mathcal{L}(M(t')) dt'
\end{equation}

A spatio-temporal metric semantic map $M(t)$ \todo{as outlined in (\ref{eq:composition}), probably best to fuse these two statements}:
\begin{gather}
    M(t) = \{ o_j(t) \} \label{eq:map_composition} \\
    o_j(t) = \{_{O_j}\Omega_j(t),\ T_{WO_j}(t)\} \label{eq:map_elements} \\
    \hat{\Omega}(t) = \sum_{M(t)} T_{WO_j}(t) * _{O_j}\Omega_j(t) \label{eq:map_surface}
\end{gather}
where the map $M$ is composed of objects $o_j$ (\ref{eq:map_composition}), each object $o_j$ has an estimated surface $_{O_j}\Omega_j(t)$ and estimated pose $T_{WO_j}(t)$ (\ref{eq:map_elements}).

For each time step $t$ where the map is queried, the goal is to recover the underlying structure $\mathcal{E}$ in the map $M$ (\ref{eq:goal_structure}). 
Additionally, we want to recover the poses of each object detected object $o_j$ that has a counterpart $e_i$ (\ref{eq:goal_poses}).
Based on computation available, we want to reconstruct the surfaces as much as possible. 
While initially $\Omega_j(0) = \emptyset \ \forall j$, we want to estimate $\Omega_j(t)$ for a selected subset $M_\Omega(t) \subseteq M(t)$ (\ref{eq:goal_surface}).

\begin{gather}
    g_s(M, t) = \lVert M(t),\ \mathcal{E}(t) \rVert \label{eq:goal_structure} \\
    g_p(M, t) = \sum_{(o_j, e_i) \in A} \lVert T_{WO_j}(t),\ T_{WE_i}(t) \rVert \label{eq:goal_poses} \\
    g_r(M, t) = \lVert \Omega(t),\ \hat{\Omega} \rVert \label{eq:goal_surface}
\end{gather}

where $\lVert\cdot\rVert$ is some similarity measure \todo{We'll put some actual metrics, or at least later in the experimental setup section}.
This yields the map quality function:

\begin{equation}
   \mathcal{L}(M(t')) = \alpha_s g_s(M(t')) + \alpha_p g_p(M(t')) + \alpha_r g_r(M(t'))
\end{equation}
Where $\alpha$ emphasize the importance of the different components.
\note{Could also say something about not including prediction/extrapolation for now. Could also say detecting which things are moving?}
\todo{Somewhere it should say given previous measurements}

% ==============================================================================================

\section{Approach}
\label{sec:approach}

\textbf{Points for narrative:}

\subsection{Notation}
\LC{maybe we should distinguish objects and stuff (https://arxiv.org/pdf/1612.03716.pdf) or find a more general term?}
We denote the state of each object $i$ at time $t$ as $O_i^t$:
\begin{equation}
    O_i^t = \{ \Omega_i^t, \ T_{WO_i}^t, \ L_i \},
\end{equation}
where $\Omega_i^t$ denotes the surface, $T_{WO_i}^t$ the pose w.r.t. world frame $W$, $L_i$ the semantic label of $O_i$ at time $t$. \LC{do we want to have the semantics time-varying?}
% We use $E_i^t \in \{0,1\}$ to indicate whether $O_i$ \emph{exists} at time $t$, i.e. $E_i^t =1 \text{ iff. } O_i^t \in \mathcal{W}$.
% At each time step $t$, a different set of objects may exist in the area of interest.
In the following, we use the shorthand notation for indexed variables of omitting the index or time step to refer to all existing indices or time steps.%, i.e.:
% \begin{gather}
%     O_i =\{ O_i^t | E_i^t = 1\}_{t=0,\dots,T}, \quad O^t =\{ O_i^t | E_i^t = 1\}_{i=0,\dots,N_O} \\
%     O = \bigcup_{t=0}^{T} O^t = \bigcup_{i = 0}^{N_O} O_i = \{ O_i^t  | E_i^t = 1\}^{t=0, \dots, T}_{i = 0,\dots,N_O}
% \end{gather}
% Note that while $N_O$ denotes the total number of objects ever present, the number of present objects $|O^t|$ may be different for each $t$.

At each $t$ the robot observes a volume $V^t$, which gives rise to measurements $Z_j^t$:
\begin{gather}
    Z_j^t = \{ \Omega_j^t, \ T_{RZ_j}^t, \ L_j^t \}, \label{eq:measurement} \\
     Z_j^t \sim O_i^t + \eta \text{ if } O_i^t \in V^t \label{eq:measurement_distrib}
\end{gather}
\LC{we might need to add something to model occlusions/field of view}
\LC{Also: we might want to clarify if the measurement includes multiple objects or there is a measurement for each object}
where $\Omega_j^t$ is a surface measurement, e.g. a point cloud, $T_{RZ_j}^t$ is the pose w.r.t. to robot frame $R$, and $L_j$ the semantic label of $Z_j$ at time $t$.
Measurements are generated of the actual objects $O_i^t$ if they are visible, and are subject to measurement errors $\eta$ (which may include missed or hallucinated $Z_j^t$).

Lastly, we define the robot poses $X$ as:
\begin{equation}
    X = \{ X^t \}_{t=0, \dots,T}, \quad X^t = T_{WR}^t
\end{equation}

At each $t$, the robot makes a set of observations $Z^t$ and an odometry measurement $\Phi^t \sim \left(T_{WR}^{t-1}\right)^{-1}T_{WR}^{t} + \eta_\Phi$.

\yun{Personal preference with  $\Phi^t \sim \left(X^{t-1}\right)^{-1}X^{t} + \eta_\Phi$ but don't feel strongly about it.} \LC{here we need some exponential map for the noise since we cannot sum poses}


\subsection{Estimation Problem}
We thus formulate the goal of spatio-temporal metric semantic mapping (STMSM) task at each current time step $T$ as a maximum a posteriori (MAP) estimation problem:
\begin{equation}
    O^\star , X^\star = \argmax_{O, X} \p(O, X | Z, \Phi) \label{eq:estimation}
\end{equation}

However, it is important to point out that (\ref{eq:estimation}) is an extremely hard problem to solve:
\todo{Check with other hardness pointed out in next section, rephrase/unify.}
\begin{enumerate}
    \item There is a large and unknown number of variables to optimize and comparably few constraints, i.e. $|O| \sim |Z|$.
    \item The problem grows very quickly over time, as $|O|$ and $|Z|$ can grow by several hundred per second. This makes the problem harder to solve, in particular in real-time for interactive robot tasks.
    \item In order to explain all $O$, all $Z$ need to be kept in memory, leading to high memory consumption.
    \item Since objects can move and robot state beliefs $X$ can change over time, associations between $O$ and $Z$ can change frequently and be hard to establish.
\end{enumerate}
Intuitively, these reflect that changes
To overcome these limitations, we propose a novel factorization of the above problem based on the idea of \emph{spatio-temporal local consistency}.

\subsection{Assumption: Local Consistency} 
We assume that:
\begin{gather}
   \left\lVert \prod_{t'=t-\tau}^{t} \Phi^{t'}- \left( T_{WR}^{t-1} \right)^{-1}T_{WR}^{t} \right\rVert < \epsilon_s \ \forall t, \ \forall \tau < \delta \label{eq:spatial_consistency} \\
     \left\lVert O^t_i - O^{t-\tau}_i \right\rVert < \epsilon_t \ \forall t, \ \forall \tau < \delta \label{eq:temporal_consistency}
\end{gather}
Intuitively, this means that errors in state estimation (\ref{eq:spatial_consistency}) and changes in objects (\ref{eq:temporal_consistency}), while they may grow large over time, are less than a small quantity $\epsilon$ for short times $\delta$.
\todo{These are very reasonable assumptions.}
% Finally, we define the consistency $C(\cdot, \cdot)$ of each object $O_i$ as:
% \begin{equation}
%     C(O_i^0) =0, \quad C(O_i^t) = \begin{cases} 
%          C(O_i^{t-1}) & \text{if } T_{RR}^t T_{R\hat{O}_k}^t \in V^t \wedge \\
%         C(O_i^{t-1}) + 1 & \text{otherwise.}
%     \end{cases}
% \end{equation}

% ==============================================================================================
\section{Drafts}

Sources for errors:
\begin{itemize}
    \item Sensing noise
    \item state estimation drift
    \item short-term motion
    \item long-term changes
\end{itemize}
% \todo{Formalize in math (maybe w.r.t. previous definition)}

Narrative about rel work:\begin{itemize}
    \item If only one (or few) of these factors are addressed, the problem becomes much easier as factors can be isolated.
\end{itemize}

Global problem statement:
"Find the 4D map that best explains all measurements" \todo{mathify w.r.t. above definitions} $\xrightarrow{}$ intractable.

We therefore propose a factorization based on the idea of local consistency.

\parsec{Assumption: Local Consistency}
\begin{itemize}
    \item Odometry drift is low over short amount of time/distance traveled. $\xrightarrow{}$ Eliminate factor of global spatial misalignment in active window.
    \item all dynamics happen within view of the robot $\xrightarrow{}$ They are continuous (=short-term) dynamics
    \item Thus, eliminates global drift and long-term problem.
    \item Left over errors to address: short-term dynamics, segmentation errors, and measurement noise (This can be solved, in particular we make this much easier with our delayed-choice-local-optimization)
    \item Requirements: Things exit the local window when exiting the field of view (or some time/distance horizon?), otherwise consistency of local observations can not be guaranteed.
\end{itemize}

\parsec{AW Challenges}
\begin{itemize}
    \item To satisfy (TODO: Objective Eq) the robot needs estimates as soon as possible (per frame)
    \item per-frame estimates can be improved over time (what we do in AW)
    \item still constrained by semantic consistency limit, so AW is the only horizon for 'early' (=tracking) optimization (Erase FP motion detections (maybe also FN), same for semantics)
\end{itemize}

\parsec{Gobal Optimization}
\begin{itemize}
    \item Input: Segmented, locally consistent patches $\xrightarrow{}$ Can exclude measurement and short-term dynamics
    \item Left to be solved: Global alignment and long-term changes.
    \item Task made a bit easier with pre-detection of some objecst of which we know can change?
    \item Use semantic knowledge of what we know is mostly background and movable objects to guide spatial alignment, then use that for change detection?
\end{itemize}






% ==============================================================================================
\section{Existing Frameworks and Assumptions}

\parsec{Sparse Representation}
For each frame, extract a set of landmarks $L^t$ and  match or add the landmarks $l_i^t$ to the map $L$:
\begin{gather}
    L^t = \{l_i^t \} \subseteq P^t \\
    l_i^t \mapsto L = \bigcup_{\tau=0}^{t-1}L_t
\end{gather}

% -----------------------------------------------------------------------------------------------

\parsec{Dense Representation}
\todo{?}
For each frame, extract a set of landmarks $L^t$ and  match or add the landmarks $l_i^t$ to the map $L$:
\begin{gather}
    L^t = \{l_i^t \} \subseteq P^t \\
    l_i^t \mapsto L = \bigcup_{\tau=0}^{t-1}L_t
\end{gather}

% -----------------------------------------------------------------------------------------------

\subsection{Families of Tasks}
\parsec{State Estimation} 
Estimate the poses $X^\tau:= T_{WS}^\tau \ \forall \tau \leq t$:
\begin{gather}
    X = \arg\max_X \mathbb{P}(P | X)
\end{gather}

\parsec{Dense Mapping} 
Estimate the poses $X^\tau:= T_{WS}^\tau \ \forall \tau \leq t$:
\begin{gather}
    X = \arg\max_X \mathbb{P}(P | X)
\end{gather}

\parsec{Semantic Mapping} 
Estimate the poses $X^\tau:= T_{WS}^\tau \ \forall \tau \leq t$:
\begin{gather}
    X = \arg\max_X \mathbb{P}(P | X)
\end{gather}

% -----------------------------------------------------------------------------------------------

\subsection{Families of Approaches}
\parsec{Static SLAM} 
Assumptions:
\begin{itemize}
    \item $\Omega=const$
    \item Associate measurements to landmarks $P^t \mapsto L = \{l_i\}$
    \item 
\end{itemize}

\newpage


